The seven most massive clumps in W43-Main as seen by ALMA: Dynamical equilibrium and Magnetic Fields

Here we present new ALMA observations of polarized dust emission from six of the most massive clumps in W43-Main. The clumps MM2, MM3, MM4, MM6, MM7, and MM8, have been resolved into two populations of fragmented filaments. From these two populations we extracted 81 cores (96 with the MM1 cores) with masses between 0.9 \Msun\ to 425 \Msun\ and a mass sensitivity of 0.08 M$_{\odot}$. The MM6, MM7, and MM8 clumps show significant fragmentation, but the polarized intensity appears to be sparse and compact. The MM2, MM3, and MM4 population shows less fragmentation, but with a single proto-stellar core dominating the emission at each clump. Also, the polarized intensity is more extended and significantly stronger in this population. From the polarized emission, we derived detailed magnetic field patterns throughout the filaments which we used to estimate field strengths for 4 out of the 6 clumps. The average field strengths estimations were found between 500 $\mu$G to 1.8 mG. Additionally, we detected and modeled infalling motions towards MM2 and MM3 from single dish HCO$^{+}(J=4 \rightarrow 3)$ and HCN$(J=4 \rightarrow 3)$ data resulting in mass infall rates of $\dot{\mathrm{M}}_{\mathrm{MM2}} = 1.2 \times 10^{-2}$ \Msun\ yr$^{-1}$ and $\dot{\mathrm{M}}_{\mathrm{MM3}} = 6.3 \times 10^{-3}$ \Msun\ yr$^{-1}$. By using our estimations, we evaluated the dynamical equilibrium of our cores by computing the total virial parameter $\alpha_{\mathrm{total}}$. For the cores with reliable field estimations, we found that 71\% of them appear to be gravitationally bound while the remaining 29\% are not. We concluded that these unbound cores, also less massive, are still accreting and have not yet reached a critical mass. This also implies different evolutionary time-scales, which essentially suggests that star-formation in high mass filaments is not uniform.

==> ms_header.tex <==

%%%%%%%%%%%%%%
% Short cuts %
%%%%%%%%%%%%%%

% Astrometry Units

\newcommand{\hr}{\mbox{$^h$}}
\renewcommand{\min}{\mbox{$^m$}}
\renewcommand{\sec}{\mbox{$^s$}}
\renewcommand{\deg}{\mbox{$^{\circ}$}}
%\newcommand{\arcmin}{\mbox{$^'$}}
%\newcommand{\arcsec}{\mbox{$^{''}$}}
\newcommand{\kms}{\mbox{km\,s$^{-1}$}}
\newcommand{\fluxunits}{\mbox{erg\,cm$^{-2}$ s$^{-1}$}}
\newcommand{\uJy}{\mbox{$\mu$Jy}}
\newcommand{\um}{\mbox{$\mu$m}}
\newcommand{\ULL}{\mbox{$<27.0$}}
% Miscellaneous
\newcommand{\dbrk}{\mbox{$D(4000)$}}
\newcommand{\wrst}{\mbox{$W_{\lambda}^{\mbox{\tiny rest}}$}}
\newcommand{\wrsti}{\mbox{$W_{\lambda,i}^{\mbox{\tiny rest}}$}}
\newcommand{\wobs}{\mbox{$W_{\lambda}^{\mbox{\tiny obs}}$}}
\newcommand{\haln}{\mbox{H$\alpha$(n)}}
\newcommand{\halb}{\mbox{H$\alpha$(b)}}
\newcommand{\simgtr}{\, \raisebox{-.2ex}{$\stackrel{>}{\mbox{\tiny $\sim$}}$} \,}
\newcommand{\simlt}{\, \raisebox{-.2ex}{$\stackrel{<}{\mbox{\tiny $\sim$}}$} \,}
\newcommand{\sigsky}{\mbox{$\sigma_{\mbox{\tiny sky}}$}}
\newcommand{\bootes}{Bo\"{o}tes}
\newcommand{\lamfwhm}{\mbox{$\Delta \lambda_{\mbox{\tiny FWHM}}$}}
\newcommand{\lamblaze}{\mbox{$\lambda_{\mbox{\tiny blaze}}$}}
\newcommand{\rarrow}{\mbox{$\Rightarrow$}}
\newcommand{\fshrt}{\mbox{$f_{\tiny \nu}^{\mbox{\tiny short}}$}}
\newcommand{\flng}{\mbox{$f_{\tiny \nu}^{\mbox{\tiny long}}$}}
\newcommand{\ztit}{\mbox{$z \approx 4.5$}}
\newcommand{\x}{\mbox{$\times$}}
\newcommand{\Msun}{\mbox{M$_{\odot}$}}
\newcommand{\Mdot}{\mbox{$\dot{m}_{-4}$}}
\newcommand{\Lsun}{\mbox{L$_{\odot}$}}
\newcommand{\E}[1]{\hbox{$10^{ #1 }$}}
\newcommand{\per}[1]{\hbox{#1$^{-1}$}}
\newcommand{\tothe}[1]{\hbox{$^{#1}$}}
\newcommand{\about}{\mbox{$\sim$}}
\newcommand{\SIG}{\mbox{W~m$^{-2}$~Hz$^{-1}$~sr$^{-1}$}}
\newcommand{\nISM}{\mbox{$n_{\rm ISM}$}}
%\newcommand{\uJy}{\mbox{$\mu$Jy}}
%\newcommand{\about}{\mbox{$\sim$}}
\def\IRAS       {\hbox{\it IRAS}}
\def\NVSS       {\hbox{\it NVSS}}

\def\OIII       {\hbox{O\tiny{III}}}
\def\NII        {\hbox{N\tiny{II}}}
\def\NO         {\hbox{---}}
\def\HII        {\hbox{H \small{II}}}
\def\HI         {\hbox{H \small{I}}}
\def\Ha         {\hbox{H \small{$\alpha$}}}
\def\Hb         {\hbox{H \small{$\beta$}}}
\def\SFIR       {\hbox{$S_{\rm FIR}$}}
\def\HCOP       {\hbox{HCO$^{+}$}}
\def\thirCO     {\hbox{$^{13}$CO}}
\def\water      {\hbox{H$_{2}$O}}
\def\source     {\hbox{G30.79\,FIR\,10}}

